Face Recognition using Optimal Representation Ensemble

Recently, the face recognizers based on linear representations have been shown to deliver state-of-the-art performance. In real-world applications, however, face images usually suffer from expressions, disguises and random occlusions. The problematic facial parts undermine the validity of the linear-subspace assumption and thus the recognition performance deteriorates significantly. In this work, we address the problem in a learning-inference-mixed fashion. By observing that the linear-subspace assumption is more reliable on certain face patches rather than on the holistic face, some Bayesian Patch Representations (BPRs) are randomly generated and interpreted according to the Bayes' theory. We then train an ensemble model over the patch-representations by minimizing the empirical risk w.r.t the "leave-one-out margins". The obtained model is termed Optimal Representation Ensemble (ORE), since it guarantees the optimality from the perspective of Empirical Risk Minimization. To handle the unknown patterns in test faces, a robust version of BPR is proposed by taking the non-face category into consideration. Equipped with the Robust-BPRs, the inference ability of ORE is increased dramatically and several record-breaking accuracies (99.9% on Yale-B and 99.5% on AR) and desirable efficiencies (below 20 ms per face in Matlab) are achieved. It also overwhelms other modular heuristics on the faces with random occlusions, extreme expressions and disguises. Furthermore, to accommodate immense BPRs sets, a boosting-like algorithm is also derived. The boosted model, a.k.a Boosted-ORE, obtains similar performance to its prototype. Besides the empirical superiorities, two desirable features of the proposed methods, namely, the training-determined model-selection and the data-weight-free boosting procedure, are also theoretically verified.

==> alg_blrcn.tex <==
% LaTeX Source
% Author:        Hanxi Li {lihanxi2001@gmail.com}
% Creation:      Tuesday 01/03/2011 14:48.
% Last Revision: Tuesday 01/03/2011 14:48.

\begin{algorithm}[t!]
  \caption{ \footnotesize BLRC-Neighborhood}   
\footnotesize{
    \begin{enumerate}
    \itemsep -2pt
      \item Normalize the training faces $\X$ and test face $\y$.
      \item Generate $\n_p$ face neighborhoods $\mathbb{Q} = \{\mathcal{N}_1,
            \mathcal{N}_2, \cdots, \mathcal{N}_{n_l}\}$, approximately covering the
            distribution of $\X$ 
      \item Generate the associated weak classifiers $\gamma_j ~\forall j \in \{1, 2,
            \cdots, n_l\}$.
      \item Get all the predict labels $\gamma_j(\x_i)~\forall i, j$.
      \item Train the BLRC-N using SAMME.U, record the selected neighborhoods and their
            weights $\alpha_t ~t = 1, 2, \cdots, T$.
      \item Select the gallery faces according to the chosen neighborhoods and perform
            each neighborhood-based weak classifier to get $\gamma_j(\y)~\forall j$.
      \item Aggregate the predict labels using \eqref{equ:predict_blrc}.
    \end{enumerate}
  }
\label{alg:blrcn}
\end{algorithm}






==> alg_blrcp.tex <==
% LaTeX Source
% Author:        Hanxi Li {lihanxi2001@gmail.com}
% Creation:      Tuesday 01/03/2011 14:48.
% Last Revision: Tuesday 01/03/2011 14:48.

\begin{algorithm}[t!]
  \caption{ \footnotesize BLRC-Patch}   
\footnotesize{
    \begin{enumerate}
    \itemsep -2pt
      \item Normalize the training faces $\X$ and test face $\y$.
      \item Generate $\n_p$ face patches $\mathbb{P} = \{p_1, p_2, \cdots,p_{n_p}\}$ on
            the training images and the associated weak classifiers $\gamma_j ~\forall j \in \{1,
            2, \cdots, n_p\}$.
      \item Get all the predict labels $\gamma_j(\x_i)~\forall i, j$.
      \item Train the BLRC-P using SAMME, record the selected face patches and their
            weights $\alpha_t ~t = 1, 2, \cdots, T$.
      \item Crop the selected patches for $\y$ and perform each patch-based weak
            classifier, get predictions $\gamma_j(\y)~\forall j$.
      \item Aggregate the predict labels using \eqref{equ:predict_blrc}.
    \end{enumerate}
  }
\label{alg:blrcp}
\end{algorithm}






==> alg_blrcp_n.tex <==
% LaTeX Source
% Author:        Hanxi Li {lihanxi2001@gmail.com}
% Creation:      Tuesday 01/03/2011 16:15.
% Last Revision: Tuesday 01/03/2011 16:15.
\begin{algorithm}[t!]
  \caption{ \footnotesize BLRC-P, BLRC-N for facial recognition}   
\footnotesize{
    \begin{enumerate}
    \itemsep -1pt
%       \item Normalize the training faces $\X$ and test face $\y$.
      \item {\bf BLRC-P}: Generate $n$ face patches $\mathbb{P} = \{p_1, p_2,
            \cdots,p_{n}\}$ \\
            {\bf BLRC-N}: Generate $n$ neighborhoods $\mathbb{Q} = \{\mathcal{N}_1,
            \mathcal{N}_2, \cdots, \mathcal{N}_{n}\}$
      \item Generate the associated weak classifiers $\gamma_j ~\forall j \in \{1, 2,
            \cdots, n\}$.
      \item Obtain all the predict labels $\gamma_j(\x_i)~\forall i, j$.
      \item Train the recognizer using SAMME (BLRC-P) or SAMME.U (BLRC-N), record the
            selected face patches (BLRC-P) or neighborhoods (BLRC-N) and the corresponding
            weights $\alpha_t, ~t = 1, 2, \cdots, T$. 
      \item Apply each weak classifier on test face $\y$ and get predictions $\gamma_j(\y)~\forall j$.
      \item Obtain the final prediction using \eqref{equ:predict_blrc}.
    \end{enumerate}
  }
\label{alg:blrcpn}
\end{algorithm}



==> alg_samme.tex <==
% LaTeX Source
% Author:        Hanxi Li {lihanxi2001@gmail.com}
% Creation:      Sunday 20/02/2011 19:51.
% Last Revision: Tuesday 01/03/2011 10:38.


\begin{algorithm}[t!]
  \caption{ \footnotesize  SAMME: multi-class boosting}   
\footnotesize{
  \KwIn
  {
    % \begin{itemize}
    % \itemsep -2pt
    %   \item A training data-label set $(\x_1, l_1), \cdots, (\x_N, l_N)$.
    %   \item A data weight set $\omega_1, \cdots, \omega_N$.
    %   \item A functional space $\mathbb{H}$ of the weak classifier $h(\x)$.
    %   \item A maximum iteration $T$.
    % \end{itemize}
  A training data-label set $(\x_1, l_1)$, $\cdots$, $(\x_N, l_N)$; 
  A functional space $\mathbb{H}$ of the weak classifier $h(\x)$; and maximum
  iteration number $ T $. 
}
  \Begin
  {
  $\cdot$  Initialize the training sample weights: $\omega_i = 1/N,~ ~ i = 1, 2, \cdots, N$\;
    \For{$t \leftarrow 1$ \KwTo $T$}
    {
    $\cdot$  Find the best weak classifier $h_t(\x) \in \mathbb{R}$, such that
      $h_t = \argmin_{h \in \mathbb{H}}\Sum_{i = 1}^{N}\omega_i \cdot \llbracket h(\x_i)
      \ne l_i\rrbracket$\;
    $\cdot$  Compute $\varepsilon_t = \Sum_{i = 1}^{N}\omega_i \cdot \llbracket h_t(\x_i) \ne
      l_i\rrbracket/\Sum_{i = 1}^{N}\omega_i$\;
    $\cdot$ Set  $\alpha_t =  \log\left((1 - \varepsilon_t)/\varepsilon_t\right) + \log(K - 1)$\;
    $\cdot$  Set $\omega_i \leftarrow \omega_i\cdot \exp\left(\alpha_t \cdot \llbracket h_t(\x_i)
      \ne l_i\rrbracket \right)$\;
    $\cdot$  Re-normalize $\omega_i$\; 

    $\cdot$  {\bf if } converge, break\;
    }
  }
  \KwOut
  {
    % \begin{itemize}
    %   \item
          The strong classifier: $ F( \x ) =  \argmax_k \textstyle \sum_{t = 1}^{T}\alpha_t \cdot
          \llbracket h_t(\x) =
        k\rrbracket$\;
   % \end{itemize}
  }
  }
\label{alg:samme}
\end{algorithm}





==> alg_sammeu.tex <==
% LaTeX Source
% Author:        Hanxi Li {lihanxi2001@gmail.com}
% Creation:      Saturday 26/02/2011 01:19.
% Last Revision: Tuesday 01/03/2011 10:39.
\begin{algorithm}[t]
  \caption{ \footnotesize SAMME.U: SAMME with uncertain predictors}   
 \footnotesize{
  \KwIn
  {
    % \begin{itemize}
    % \itemsep -2pt
    %   \item A training data-label set $(\x_1, l_1), \cdots, (\x_N, l_N)$.
    %   \item A data weight set $\omega_1, \cdots, \omega_N$.
    %   \item A functional space $\mathbb{H} = \{\gamma_j(\x), \gamma_j(\x), \cdots,
    %     \gamma_j(\x)\}$. 
    %   \item A maximum iteration $T$.
    % \end{itemize}
    A training data-label set $(\x_1, l_1)$, $\cdots$, $(\x_N, l_N)$; 
  A functional space $\mathbb{H}$ of the weak classifier $h(\x)$; and maximum
  iteration number $ T $.     
    }
  \Begin
  {
  $\cdot$  Initialize the weights $\omega_i = 1/N,~ ~ i = 1, 2, \cdots, N$\;
    \For{$t \leftarrow 1$ \KwTo $T$}
    {
    $\cdot$  Fit the weak classifier $\gamma_t(\x) \in \mathbb{R}$, such that
      $\gamma_t = \argmin_{\gamma \in \mathbb{H}}\Sum_{i = 1}^{N}\omega_i \cdot
      \Psi(\x_i)$\;
    $\cdot$  Compute $\varepsilon_t$ by using \eqref{equ:sammeu_werr}\;
      $\alpha_t \leftarrow \log((1 - \varepsilon_t)/\varepsilon_t) + \log(K - 1)$\;
    $\cdot$  Set $\omega_i \leftarrow \omega_i\cdot \exp\left(\alpha_t \cdot \Psi(\x_i) \right)$\;
    $\cdot$  Re-normalize $\omega_i$\;

    $\cdot$  {\bf if } converge, break\;


    }
  }
  \KwOut
  {
  The strong classifier: 
   $F(\y) = \argmax_k\sum_{t = 1}^{T}\alpha_t \cdot \llbracket \gamma_t(\y)
        = k\rrbracket$\;
   }
  }
\label{alg:sammeu}
\end{algorithm}





==> tab_feret_recog_accuracy.tex <==
% ******************** Generated by LatexTableGenerator ********************
    \begin{table}[h]
    \centering
    \resizebox{0.48\textwidth}{!}
    {
    \begin{tabular}{ l | l | l | l | l | l | l }

    \hline\hline
    % List the column names as follows.
&   & D-40    & D-50    & D-100    & D-200    & D-300   \\
\cline{1-7}
{\bf \multirow{3}{*}{Random}}  
& LRC  & $62.0\pm2.3$  & $68.7\pm4.0$  & $74.3\pm2.0$  & $76.0\pm2.6$  & $77.5\pm2.8$  \\
& SRC  & $67.5\pm3.1$  & $70.6\pm2.6$  & $74.0\pm1.6$  & $73.0\pm2.0$  & $72.5\pm2.8$  \\
& NFL  & $70.1\pm4.3$  & $72.1\pm3.4$  & $75.8\pm2.3$  & $76.4\pm3.6$  & $77.7\pm2.2$  \\
\cline{1-7}
{\bf \multirow{3}{*}{Eigen}}  
& LRC  & $79.6\pm3.1$  & $79.4\pm3.5$  & $79.7\pm1.9$  & $79.3\pm2.3$  & $78.2\pm2.6$  \\
& SRC  & $78.2\pm2.1$  & $79.2\pm2.8$  & $78.7\pm1.6$  & $75.9\pm2.1$  & $74.0\pm2.1$  \\
& NFL  & $78.2\pm2.8$  & $78.5\pm3.0$  & $78.2\pm3.0$  & $78.3\pm2.7$  & $78.5\pm2.6$ \\
\cline{1-7}
\multicolumn{2}{c|}{\bf{BLRC-N}}  & \multicolumn{5}{c}{$\bf 81.2\pm1.5$}  \\
\multicolumn{2}{c|}{\bf Sampling} & \multicolumn{5}{c}{$79.8\pm3.0$} \\  
    \hline\hline
    \end{tabular}
    }
    \caption
    {
        Comparison of recognition results on the FERET dataset.  Sampling means randomly
        selecting a subset the entire training samples to build LRC classifiers and vote
        for the final result. We don't perform the test with $20$-D face features because
        LRC requires the dimension of the feature larger than the number of training
        images belonging to one individual.
    }
    \label{tab:feret_accuracy}
    \end{table}

% ******************** Generated by LatexTableGenerator ********************


